Resilient Distributed Vector Consensus Using Centerpoints

In this paper, we study the resilient vector consensus problem in networks with adversarial agents and improve resilience guarantees of existing algorithms. A common approach to achieving resilient vector consensus is that every non-adversarial (or normal) agent in the network updates its state by moving towards a point in the convex hull of its \emph{normal} neighbors' states. Since an agent cannot distinguish between its normal and adversarial neighbors, computing such a point, often called as \emph{safe point}, is a challenging task. To compute a safe point, we propose to use the notion of \emph{centerpoint}, which is an extension of the median in higher dimensions, instead of Tverberg partition of points, which is often used for this purpose. We discuss that the notion of centerpoint provides a complete characterization of safe points in $\mathbb{R}^d$. In particular, we show that a safe point is essentially an interior centerpoint if the number of adversaries in the neighborhood of a normal agent $i$ is less than $\frac{N_i}{d+1} $, where $d$ is the dimension of the state vector and $N_i$ is the total number of agents in the neighborhood of $i$. Consequently, we obtain necessary and sufficient conditions on the number of adversarial agents to guarantee resilient vector consensus. Further, by considering the complexity of computing centerpoints, we discuss improvements in the resilience guarantees of vector consensus algorithms and compare with the other existing approaches. Finally, we numerically evaluate the performance of our approach through experiments.

==> Automatica (Resilient Vector Consensus using Centerpoint)/Evaluation.tex <==
\section{Numerical Evaluation}
\label{sec:Evaluation}
We perform simulations to illustrate resilient consensus in multirobot systems in two dimensions using centerpoint, and compare it with the one using approximate Tverberg partition \cite{park2017fault}.\footnote{Our code is available at \url{https://github.com/JianiLi/MultiRobotsRendezvous}} We model interconnections between robots using the following graphs: %(for different experiments):

\begin{itemize}
    \item A disk graph $\mathcal{G}_d = (\mathcal{V}, \mathcal{E}(t))$, in which each node $i\in\mathcal{V}$ (representing a robot) has a sensing radius $r$ and $(j,i)\in\mathcal{E}(t)$ if and only if $||x_j(t) - x_i(t)|| \le r$.  
    \item A fixed {undirected} graph $\mathcal{G} = (\mathcal{V}, \mathcal{E})$ whose edge set does not change over time.
\end{itemize}

At each iteration $t$ of the consensus algorithm, a normal robot $i$ computes an $F_i$-safe point $s_i(t)$ of its neighbors' positions (using centerpoint or approximate Tverberg partition), and calculates its new position using \eqref{eq:ADRC}. In our experiments, we set $\alpha_i(t) = 0.8$, for all $t$.

%Next, it calculates the next position, $ x_i(t+1) = x_i(t) + u_i(t)$, where $u_i(t) = \alpha_i(t)(s_i(t) - x_i(t))$. Here, $\alpha_i(t)$ controls the velocity of robots. If the control vector $u_i(t)$ is smaller than a threshold $\delta$, then the robot halts, otherwise, it executes the control. In our experiments, we set $\alpha_i(t) = 0.8$ and $\delta = 0.001$ for all normal robots.

%--------------------------- subsection begins --------
\subsection{Centerpoint based resilient consensus}
We simulate a group of 120 robots, {out of which 100 are normal and 20 are adversarial}. They are deployed in a planar region $\mathcal{W} = [-1,1] \times [-1,1] \in \mathbb{R}^2$ as shown in \figref{fig: centerpoint consensus initial topology}(a), where nodes in blue are normal robots executing consensus and nodes in red represent adversarial robots. We consider three types of adversarial behaviors:
\begin{itemize}
    \item \emph{Stationary} -- each red node has a fixed position that does not change throughout the simulation.
    \item \emph{Oscillating} -- each red node changes its position by moving from corner to corner within the square of length 0.1, as depicted in \figref{fig: centerpoint consensus initial topology}(b).
    \item \emph{Move-away} -- each red node moves towards the closest corner of the region $\mathcal{W}$ from its initial position % with a step size $|u_i(t)(0)| = 0.1$ and $|u_i(t)(1)| = 0.1$ 
    and then stays there, as shown in \figref{fig: centerpoint consensus initial topology}(c).
    %and stays stationary at the corner if the next move will make it escape from $\mathcal{W}$, as shown in \figref{fig: centerpoint consensus initial topology}(c).
\end{itemize}


The interconnection topology is captured by a disk graph with a fixed sensing radius of $r = 0.45$ for every normal robot. Each normal robot executes consensus algorithm based on centerpoint. Consensus is guaranteed if the number of adversarial robots in the neighborhood of each normal robot $i$ is $F_i \le \left(\left\lfloor \frac{{N}_i}{3}\right\rfloor-1\right)$ \textcolor{blue}{and the sequence of graphs induced by normal agents is repeatedly reachable. Both of these conditions are satisfied in all the simulations here.} Consequently, normal robots achieve consensus in the presence of all three types of adversarial nodes, as shown in Figures \ref{fig: centerpoint consensus evolution} and \ref{fig: centerpoint consensus positiion change}.
%Moreover, \figref{fig: centerpoint consensus positiion change} shows positions (both $x$ and $y$ coordinates) of normal robots as a function of iterations.


%---------- New Figure Begins ---------
\begin{figure}[htb]
\centering
\begin{subfigure}[b]{0.155\textwidth}
\centering
\includegraphics[scale = 0.14]{figure/centerpoint_consensus/a.png}
\caption{}
\end{subfigure}
\begin{subfigure}[b]{0.155\textwidth}
\centering
\includegraphics[scale = 0.14]{figure/centerpoint_consensus/b.png}
\caption{}
\end{subfigure}
\begin{subfigure}[b]{0.155\textwidth}
\centering
 \includegraphics[scale = 0.14]{figure/centerpoint_consensus/c.jpg}
\caption{}
\end{subfigure}
\caption{Robots' initial positions with (a) stationary, (b) oscillating  and (c) move-away adversaries.}
\label{fig: centerpoint consensus initial topology}
\end{figure}
%---------- New Figure Ends -----------


%---------- New Figure Begins ---------
\begin{figure}[htb]
\centering
\begin{subfigure}[b]{0.155\textwidth}
\centering
\includegraphics[scale = 0.14]{figure/centerpoint_consensus/c_a.png}
\caption{}
\end{subfigure}
\begin{subfigure}[b]{0.155\textwidth}
\centering
\includegraphics[scale = 0.14]{figure/centerpoint_consensus/c_b.png}
\caption{}
\end{subfigure}
\begin{subfigure}[b]{0.155\textwidth}
\centering
 \includegraphics[scale = 0.14]{figure/centerpoint_consensus/c_c.png}
\caption{}
\end{subfigure}
\caption{Robots' positions after consensus with (a) stationary, (b) oscillating, and (c) move-away adversaries.}
\label{fig: centerpoint consensus evolution}
\end{figure}
%---------- New Figure Ends -----------

%---------- New Figure Begins ---------
\begin{figure}[htb]
\centering
\begin{subfigure}[b]{0.155\textwidth}
\centering
\includegraphics[width=1.1in, height = 1.7in, trim=0.4cm 0.4cm 0.4cm 0.4cm]{figure/centerpoint_consensus/cstat.png}
\caption{}
\end{subfigure}
\begin{subfigure}[b]{0.155\textwidth}
\centering
 \includegraphics[width=1.1in, height = 1.7in, trim=0.4cm 0.4cm 0.4cm 0.4cm]{figure/centerpoint_consensus/cosc.png}
\caption{}
\end{subfigure}
\begin{subfigure}[b]{0.155\textwidth}
\centering
\includegraphics[width=1.1in, height = 1.7in, trim=0.4cm 0.4cm 0.4cm 0.4cm]{figure/centerpoint_consensus/cmove.png}
\caption{}
\end{subfigure}
\caption{Normal robots' positions as functions of iterations in the case of (a) stationary, (b) oscillating, and (c) move-away adversaries.}
\label{fig: centerpoint consensus positiion change}
\end{figure}
%---------- New Figure Ends -----------


%--------------------------- subsection begins --------
\subsection{Comparison of Approximate Tverberg Partition and  Centerpoint-based Resilient Consensus}
To demonstrate the improved resilience of centerpoint-based consensus compared to the Tverberg partition-based one, we consider stationary adversarial nodes and assume that the network graphs are fixed. In our first example, we consider a group of 28 robots deployed in a planar region $\mathcal{W} = [-1.5,1.5] \times [-0.375, 0.375] \in \mathbb{R}^2$ as shown in \figref{fig: simple: Robots position evolution}. There are six adversarial nodes (red) on the left and six on the planar region's right side. At the same time, 16 normal robots (blue) are divided equally into two clusters in the middle part of the region, each containing eight robots. All of the 16 normal robots are pair-wise adjacent to each other. Moreover, each normal robot is adjacent to six adversarial robots located on its side. Figures \ref{fig: simple: Robots position evolution} shows the evolution of robots' positions using approximate Tverberg partition-based and centerpoint-based consensus algorithms. As illustrated, the approximate Tverberg partition-based algorithm fails to make the normal robots converge to one point, but the centerpoint-based algorithm succeeds. The main reason is that each normal robot $i$ has {${N}_i=22$ robots in its neighborhood} (including the robot itself), of which $6$ are adversarial. The approximate Tverberg partition-based algorithm is resilient to $\left( \left\lceil \frac{{N}_i}{4}\right\rceil - 1 \right) = 5$ adversaries, % in the neighborhood of a normal node, 
whereas the centerpoint based algorithm is resilient to $\left(\left\lfloor \frac{{N}_i}{3}\right\rfloor -1\right) = 6$ adversaries. %This simple example shows that the improved resilience of centerpoint based algorithm as compared to the approximate Tverberg partition based algorithm.


%---------- New Figure Begins ---------
\begin{figure}[htb]
\centering
\begin{subfigure}[b]{0.23\textwidth}
\centering
 \centering
        \includegraphics[width=1.75in]{figure/simple/tver0}\\
        \includegraphics[width=1.75in]{figure/simple/tver1}\\
        \includegraphics[width=1.75in]{figure/simple/tver20}\\
        \caption{}
\end{subfigure}
\begin{subfigure}[b]{0.23\textwidth}
\centering
        \includegraphics[width=1.75in]{figure/simple/center0}\\
        \includegraphics[width=1.75in]{figure/simple/center5}\\
        \includegraphics[width=1.75in]{figure/simple/center20}\\
\caption{}
\end{subfigure}
\caption{The evolution of robots' positions (from top to down) in the case of (a) approximate Tverberg partition-based and the (b) centerpoint-based algorithms.}
\label{fig: simple: Robots position evolution}
\end{figure}
%---------- New Figure Ends -----------
\begin{comment}
Next, we consider a larger network in a planar region $\mathcal{W} = [-1,1] \times [-1,1] \in \mathbb{R}^2$ containing 45 robots, of which 5 are adversarial as shown in \figref{fig: 45 nodes: configuration}(a). All normal robots have at most $\left(\left\lfloor \frac{{N}_i}{3}\right\rfloor -1\right)$ adversaries in their neighborhoods, which means resilient consensus is guaranteed by the centerpoint-based algorithm. {However, a couple of normal robots (depicted in yellow color) have $F_i$ adversaries in their neighborhoods, where $ \left(\left\lceil \frac{{N}_i}{4}\right\rceil -1\right) < F_i \le \left(\left\lfloor \frac{{N}_i}{3}\right\rfloor -1\right)$.} The top and bottom yellow robots have 7 and 8 robots in their neighborhoods, respectively. Further, each yellow robot has two adversarial neighbors. 
%{For the two robots in yellow, they have 7 and 8 neighbors, %such that $\lceil \frac{|\mathcal{N}_i|}{4}\rceil -1 = 1$ for both.
%and both of them have 2 adversarial neighbors in their respective neighborhoods.} 
Consequently, the resilient consensus condition for the approximate Tverberg partition-based algorithm is not satisfied, and consensus is not guaranteed. Figures \ref{fig: 45 nodes: configuration} shows final positions of robots for both algorithms, and Figure \ref{fig: nodes 45 example position change} illustrates positions of robots as functions of iterations. It is clear that consensus is achieved with the centerpoint-based algorithm, whereas robots fail to converge at a common point using the approximate Tverberg partition-based algorithm.

%---------- New Figure Begins ---------
\begin{figure}[htb]
\centering
\begin{subfigure}[b]{0.155\textwidth}
\centering
\includegraphics[width=1in, trim=0.4cm 0.4cm 0.4cm 0.4cm]{figure/45nodes/tver0.eps}
\caption{}
\end{subfigure}
\begin{subfigure}[b]{0.155\textwidth}
\centering
 \includegraphics[width=1in, trim=0.4cm 0.4cm 0.4cm 0.4cm]{figure/45nodes/tver55.eps}
\caption{}
\end{subfigure}
\begin{subfigure}[b]{0.155\textwidth}
\centering
 \includegraphics[width=1in, trim=0.4cm 0.4cm 0.4cm 0.4cm]{figure/45nodes/center55.eps}
\caption{}
\end{subfigure}
\caption{(a) Initial positions of robots. (b) Final positions of robots using approximate Tverberg partition-based algorithm. (c) Final positions using centerpoint-based algorithm.}
\label{fig: 45 nodes: configuration}
\end{figure}
%---------- New Figure Ends -----------

%---------- New Figure Begins ---------
\begin{figure}[htb]
\centering
\begin{subfigure}[b]{0.2\textwidth}
\centering
\includegraphics[width=1.4in, height=1.9in]{figure/45nodes/comp_tv.png}
\caption{}
\end{subfigure}
\begin{subfigure}[b]{0.2\textwidth}
\centering
 \includegraphics[width=1.4in, height=1.9in]{figure/45nodes/comp_center.png}
\caption{}
\end{subfigure}
    \caption{Positions of normal robots as a function of iterations using (a) approximate Tverberg partition-based, and (b) centerpoint-based algorithms.}
    \label{fig: nodes 45 example position change}
\end{figure}
%---------- New Figure Ends -----------

\end{comment}



==> Automatica (Resilient Vector Consensus using Centerpoint)/revision1_conditions_for_safepoints.tex <==
%=========================== Subsection ======================
\subsection{Necessary Condition for $F_i$-Safe Point}
%\textcolor{red}{Waseem will add a citation of Ntin's paper. Mudassir will add that such examples have been studied in discrete geometry literature and are pretty useful/standard.}
We note that $\frac{1}{d+1} $ is the best possible fraction (for $F_i$) in Theorem \ref{thm:safe_center}, that is, there exist general node positions where allowing more adversary nodes would mean that there is no safe point at all. For example, consider a set of three points $a,b,c,$ in $\mathbb{R}^2$ that lie on the vertices of a non-degenerate triangle.\footnote{A non-degenerate triangle has three points that do not all lie on a line.} If one of these points is malicious then there is no $1$-safe point in the plane. Clearly, no point in the interior of the triangle can be $1$-safe because it does not lie in the convex hull of normal points for any choice of point corresponding to an adversary. Similarly, any point that lies on an edge of the triangle, say $\overline{ab}$, can not be $1$-safe because if one of the endpoint, say $a$, is adversarial then the convex hull of the remaining points $b$ and $c$ does not contain this point. Now in $\mathbb{R}^3$, consider four points $a,b,c,d,$ lying on the vertices of a non-degenerate tetrahedron. Assume one of these points, whose identity is unknown, is adversarial. {A point $x$ in the interior of tetrahedron} can not be $1$-safe because if $a$ is malicious then {$x$} is not contained in the convex hull of normal points $b, c ,d$, as shown in Figure~\ref{fig:NC}(a). Similarly, consider a point $x$ that lies on a facet, say $a,b,c$, of the tetrahedron. The point $x$ can not be $1$-safe because if one of the points on \textcolor{blue}{its} facet, say $b$, is adversarial then $x$ is not in the convex hull of the remaining points $a,c,d$, as shown in Figure~\ref{fig:NC}(b). In the following, we show that this example can generalized to arbitrary number of points and arbitrary dimension.

%-------------- Proposition and Proof Ends --------------------

\begin{figure}[htb]
	\centering
	\begin{subfigure}[b]{0.236\textwidth}
		\centering
		\includegraphics[scale=0.3]{single_nec_1.pdf}
		\caption{}
	\end{subfigure}
	\begin{subfigure}[b]{0.236\textwidth}
		\centering
		\includegraphics[scale=0.3]{single_nec_2.pdf}
		\caption{}
	\end{subfigure}
	\caption{An example of $4$ points in $\mathbb{R}^3$. (a)~A point $x$ in the interior of tetrahedron can not be $1$-safe because if $a$ is adversarial, then $x$ is not contained in the convex hull of the normal points. (b)~If a point $x$ lies on facet, say $a,b,c$, and $b$ is adversarial, then $x$ is not contained in the convex hull of normal point $a,c,d$. }
	\label{fig:NC}
\end{figure}

%-------------- Proposition and Proof Begins -----------------
\begin{proposition}
\label{prop:center_nec}
For a set of $N_i$ nodes in general positions, if  $F_i\ge \left\lceil \frac{N_i}{d+1} \right\rceil $, then there exist general examples in which an $F_i$-safe point does not exist.
\end{proposition}
\emph{Proof:} 
Let $a_1,a_2,\ldots,a_{d+1}$ be points that lie on the vertices of a non-degenerate $d$-simplex in $\mathbb{R}^d$ where one of the points is adversarial. A point in the interior of simplex can not be $1$-safe because it does not lie in the convex hull of normal points for an arbitrary choice of adversarial point. Consider a point $x$ that lies on a facet of $d$-simplex defined by, say, points $a_1,a_2,\ldots,a_{d}$. If one of the points, say $a_1$, on the vertices of such a facet is adversarial, then point $x$ can not lie on $(d-1)$-simplex or the convex hull of the remaining points, $a_2,a_3,\ldots,a_{d+1}$. Thus, such a point can not be a $1$-safe point.

Now, if we replace each point on a vertex of $d$-simplex by $\frac{N_i}{d+1}$ points (for simplicity, we assume $N_i$ to be a multiple of $d+1$), then we get a total of $N_i$ points that are clustered on $d+1$ vertices. {Any point $x$ in the interior of simplex} can not be  $\frac{N_i}{d+1}$-safe because if all $\frac{N_i}{d+1}$ points on an arbitrary vertex of the simplex are adversarial, then the convex hull of the remaining points does not contain {the point $x$}. Let us say we choose a point $x$ on a facet of the  $d$-simplex. If $\frac{N_i}{d+1}$ points lying on a vertex of this facet are adversarial, then the convex hull of the remaining points does not contain $x$. Thus, no point $x$ can be an $\frac{N_i}{d+1}$-safe point for this configuration of points. It is easy to see that argument still works if instead of placing all $\frac{N_i}{d+1}$ points on a vertex of $d$-simplex, we place them arbitrary close to the vertex. Thus, the statement holds for points in general positions as well. $\qed$

We note that our proof for the necessary condition for the existence of an $F_i$-safe point is based on the proof of the Centerpoint Theorem's sharpness. Similar constructions of extreme examples of pointsets are well-studied in the literature \cite{mustafa2015k,Neumann1945OnAI}.  %which is folklore in the Discrete Geometry literature.
%-------------- Proposition and Proof Ends --------------------

% \begin{figure}[htb]
% 	\centering
% 	\begin{subfigure}[b]{0.236\textwidth}
% 		\centering
% 		\includegraphics[scale=0.3]{NNCC_2.pdf}
% 		\caption{}
% 	\end{subfigure}
% 	\begin{subfigure}[b]{0.236\textwidth}
% 		\centering
% 		\includegraphics[scale=0.3]{NNCC_1.pdf}
% 		\caption{}
% 	\end{subfigure}
% 	\caption{An example of $20$ points in $\mathbb{R}^3$ is shown. Five points are placed arbitrarily close to each of the four vertices $a,b,c,d$ of a tetrahedron shape. A point $x$ in the interior of tetrahedron can not be $5$-safe because if five points near vertex $a$ are malicious then $x$ is not contained in the convex hull of the normal points as shown in (a). If a point $x$ lies on  facet, say, $a,b,c$ and points near vertex $b$ are malicious then $x$ is not contained in the convex hull of normal point near vertices $a,c,d$  as shown in (b). }
% 	\label{fig:NC}
% \end{figure}


%============= Section: d > 8 (Suff. Condition) ==============
\subsection{Sufficient Condition for $F_i$-Safe Point in Arbitrary Dimension}

In the previous section, we showed that if there are \textcolor{blue}{at least} $\lceil \frac{N_i}{d+1} \rceil$ adversarial nodes, then an $F_i$-safe point \textcolor{blue}{does not exist. In this section, we show that for \emph{any} $d$, if the number of adversarial nodes $F_i$ is less than $\lfloor\frac{N_i}{d+1}\rfloor$, then an $F_i$-safe point always exists. The main idea will be to show that for a set $\mathcal{S}$ of $N_i$ points in $\mathbb{R}^d$, there exists an interior point of depth $\lfloor\frac{N_i}{d+1}+1\rfloor$. In other words, there exists an interior point in the intersection of all convex sets containing at least $\lfloor\frac{N_i}{d+1}+1\rfloor$ points of $\mathcal{S}$. For this, we first prove some intermediate results.}


% In this section, we show that if there are fewer adversarial nodes, then we can always find an $F_i$-safe point.
% In particular, we want to prove the following theorem.}

% \begin{theorem}
% \label{thm:main_suff_con}
% \textcolor{blue}{
% For a set of $N_i$ nodes in general positions in $\mathbb{R}^d$, if  the number of adversarial nodes is less than $ \lfloor \frac{N_i}{d+1} \rfloor $, then there always exists  an $F_i$-safe point.
% }
% \end{theorem}

% The above result will be a direct consequence of Theorem~\ref{thm:general_suff} that we will prove later in this subsection. First, we state the following lemma:

%------------- Lemma and Proof Begins -------------
\begin{lemma}
\label{lem:halfspaces}
Let $\calS$ be a set of $N$ points in $\mathbb{R}^d$ in general positions, where $d\ge 1$. For a set of $d+1$ convex sets each containing at least $\lceil \frac{Nd}{d+1}+1 \rceil$ points from $\calS$, there are at least $d+1$ points of $\calS$ contained in the intersection of all halfspaces. 
\end{lemma}

\emph{Proof: } Let $X_1,X_2,\ldots,X_{d+1}$ be the convex sets, each containing at least $k$ points of $\calS$. We will refer to the number of points of $\calS$ contained in a set $X_i$ as the \textit{size} of set $X_i$ and denote it as $|X_i|$. Now, for the first set  $X_1$ we have,
	$$
	|X_1| \ge k.
	$$
	Since there are only $N-k$ points left, the set $X_2$ must contain at least $k-(N-k)$ points from $X_1$. Thus,
	$$
	|X_1\cap X_2| \ge 2k-N.
	$$
	Similarly, $X_3$ must contain at least $k-(N-|X_1\cap X_2|)$ points from $X_1\cap X_2$, that is,
	$$
	|X_1\cap X_2\cap X_3| \ge 3k-2N.
	$$
	In general, we have, 
	$$
	|X_1\cap X_2\cap \ldots X_i| \ge k-(N-|X_1\cap X_2\cap \ldots X_{i-1}|).
	$$
	It follows that,
	$$
	|X_1\cap X_2\cap \ldots X_{d+1}| \ge (d+1)k-dN.
	$$
	Substituting the value of $k$, we get the following,
	$$
	|X_1\cap X_2\cap \ldots \cap X_{d+1}| \ge (d+1)\left\lceil \frac{Nd}{d+1}+1 \right\rceil-dN.
	$$
	It follows that
	$$
	|X_1\cap X_2\cap \ldots X_{d+1}| \ge d+1,
	$$
	which is the desired claim. $\qed$

%------------- Lemma and Proof Ends -------------
The above lemma implies that any $d+1$ convex sets, each of which contains \textit{enough} points from a set $\calS$, must contain at least $d+1$ points from the same set. Now, if the original pointset $\calS$ is in general position, then so must be the $d+1$ points contained in all convex sets. Furthermore, every $d+1$ points in general positions span a $d$-simplex that contains a ball of radius $\epsilon$ in its interior for sufficiently small value of $\epsilon>0$. Thus, we get the following:

%------------- Corollary Begins -------------
\begin{corollary}
\label{cor:gen_suff}
	Let $\calS$ be a set of $N$ points in $\mathbb{R}^d$ in general positions, where $d\ge 1$. For a set of $d+1$ convex sets each containing at least $\left\lceil \frac{Nd}{d+1}+1 \right\rceil$ points from $\calS$, there exists $\epsilon>0$ such that the intersection of all convex sets contains a ball of radius $\epsilon$. 
\end{corollary} 
%------------- Corollary Ends -------------
Next, we state the following version of \emph{Helly's Theorem} \cite{klee1953critical} that will be used in the proof of Theorem \ref{thm:general_suff}.

%------------- Theorem Begins -------------
\begin{theorem}\cite{klee1953critical}
	\label{theorem:ihelly}
	If $\mathcal{K}$ is a finite family of convex sets (or an infinite family of compact convex sets) in $\mathbb{R}^d$, $C$ is a convex set such that for every $d+1$ members of $\mathcal{K}$, there exists a translate\footnote{For a set $C \subset \mathbb{R}^d$, a translate of $C$ is the set $\{c+x: c\in C\}$ for some vector $x\in \mathbb{R}^d$.} of $C$ contained in their intersection, then there is a suitable translate of $C$ contained in the intersection of all sets in $\mathcal{K}$.
\end{theorem}
%------------- Theorem Ends -------------

Now we state a crucial result to prove a sufficient condition for an $F_i$-safe point in arbitrary $d$.
%------------- Theorem and Proof Begins -------------
\begin{theorem}
\label{thm:general_suff}
For any set $\calS$ of $N$ points in $\mathbb{R}^d$ in general positions, where $d \ge 1 $, there exists an interior point in the intersection of all convex sets containing at least $\left\lceil \frac{Nd}{d+1}+1 \right\rceil$ points of $\calS$.%\footnote{\textcolor{blue}{Centerpoint Theorem implies that this bound is sharp up to $+1$.}}
\end{theorem}

\emph{Proof:} From Lemma~\ref{lem:halfspaces} and Corollary~\ref{cor:gen_suff}, we know that every $d+1$ convex sets contain an $\epsilon$ radius ball for some $\epsilon>0$. Let $\epsilon_0$ be the minimum over all such $\epsilon$ for all choices of $d+1$ convex sets.\footnote{In general, there are infinitely many such sets but we observe that any such set must contain convex hull of some $d+1$ points. Thus, it suffices to only consider $n\choose d+1$ convex sets, i.e., the convex hulls of any $d+1$ points.} Let $C$ be a ball of radius $\epsilon_0$, and let $\mathcal{K}$ be the family of all convex sets that contain points of $\calS$. Then every $d+1$ members of $\mathcal{K}$ contain a translate of $C$. It follows from Theorem~\ref{theorem:ihelly} that a suitable translate of $C$ is contained in the intersection of all sets in $\mathcal{K}$. Since $C$ is a ball of non-zero radius, it has an interior. It follows that intersection of every convex set that contains points from $\calS$ contains a ball with an interior. $\qed$

%------------- Theorem and Proof Ends -------------
\textcolor{blue}{Next, we present the main result in this subsection, that is, a sufficient condition for the existence of an $F_i$-safe point in an arbitrary dimension $d$.}

%------------- Theorem and Proof Begins -------------
\begin{theorem}
\label{thm:main_suff_con}
\textcolor{blue}{
For a set of $N_i$ nodes in general positions in $\mathbb{R}^d$, if  the number of adversarial nodes is less than $ \lfloor \frac{N_i}{d+1} \rfloor $, then there always exists  an $F_i$-safe point.
}
\end{theorem}

\textcolor{blue} {
\emph{Proof:} From the assumption of Theorem~\ref{thm:main_suff_con}, we have a set of $N_i$ points in general position of which there are less than  $\lfloor \frac{N_i}{d+1} \rfloor $ adversarial. If we take the convex hull of the remaining points, such of convex hull will contain at least $N_i - \left( \lfloor \frac{N_i}{d+1} \rfloor -1 \right) $ normal points. A family $\calK$ of convex sets each of which contains at least $\left\lceil \frac{N_id}{d+1}+1 \right\rceil$ points from a given set of $N_i$ must include the one that contains the convex hull of normal points. Theorem~\ref{thm:general_suff} states that there is a point in the interior of the intersection of family $\calK$. Therefore, existence of an interior point in the convex hull normal points, i.e., an $F_i$-safe point, is implied. This completes the proof. $\qed$
}
%------------- Theorem and Proof Ends -------------

